Test Smell Detection Tools: A Systematic Mapping Study

Test smells are defined as sub-optimal design choices developers make when implementing test cases. Hence, similar to code smells, the research community has produced numerous test smell detection tools to investigate the impact of test smells on the quality and maintenance of test suites. However, little is known about the characteristics, type of smells, target language, and availability of these published tools. In this paper, we provide a detailed catalog of all known, peer-reviewed, test smell detection tools. We start with performing a comprehensive search of peer-reviewed scientific publications to construct a catalog of 22 tools. Then, we perform a comparative analysis to identify the smell types detected by each tool and other salient features that include programming language, testing framework support, detection strategy, and adoption, among others. From our findings, we discover tools that detect test smells in Java, Scala, Smalltalk, and C++ test suites, with Java support favored by most tools. These tools are available as command-line and IDE plugins, among others. Our analysis also shows that most tools overlap in detecting specific smell types, such as General Fixture. Further, we encounter four types of techniques these tools utilize to detect smells. We envision our study as a one-stop source for researchers and practitioners in determining the tool appropriate for their needs. Our findings also empower the community with information to guide future tool development.

==> Tables/AlternativeTerms.tex <==
\begin{table}[h!]
\centering % used for centering table
\caption{List of Test Smells with Alternative Terms} % title of Table

\resizebox{\columnwidth}{!}{%
\begin{tabular} {|l|l|}\hline

\rowcolor{gray!60}
 \textbf{Test Smell} & \textbf{Alternative Terms} \\ [0.5ex]
% inserts table
%heading
\hline % inserts single horizontal line
Redundant Print	 &   Print Statement \\ % inserting body of the table

%%%%%%%%%%
\rowcolor{gray!30}
Duplicated Code	 &   TestCodeDuplication\\ 

%%%%%%%%%%

Assertionless & Assertion-Free\\
%%%%%%%%%%
\rowcolor{gray!30}
Exception Handling  & Exception Catching Throwing\\
\hline %inserts single line
\end{tabular}
}
\label{table:alternative_Terms} % is used to refer this table in the text
\end{table}


==> Tables/AuthorsTable.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h!]
\centering
\resizebox{\columnwidth}{!}{%
% \begin{adjustbox}{width=0.6\textwidth,center}

\begin{tabular} {|c|c|c|}\hline

\rowcolor{gray}
\textbf{Author} & \textbf{\# Studies} & \textbf{Ref} \\ \hline


\textbf{Fabio Palomba}           & 8   &  \cite{tufano2016empirical, palomba2016diffusion, palomba2017does, palomba2018automatic, spadini2018relation, peruma2019distribution, grano2019scented, palomba2019smell}  \\ \hline
%%%%%
\rowcolor{lightgray}
\textbf{Andrea De Lucia}         & 6   &  \cite{bavota2012empirical, bavota2015test, tufano2016empirical, palomba2016diffusion, palomba2018automatic, grano2019scented}  \\ \hline
%%%%%
\textbf{Andy Zaidman}            & 5   &  \cite{greiler2013strategies, palomba2017does, palomba2018automatic, spadini2018relation, palomba2019smell}  \\ \hline
%%%%%
\rowcolor{lightgray}
\textbf{Rocco Oliveto}           & 4   &  \cite{bavota2012empirical, bavota2015test, tufano2016empirical, palomba2016diffusion}  \\ \hline
%%%%%
\textbf{Dario Di Nucci}          & 4   &  \cite{palomba2016diffusion, de2019assessing, de2019socrates, grano2019scented}  \\ \hline
%%%%%
\rowcolor{lightgray}
\textbf{Bart Van Rompaey}        & 3   &  \cite{breugelmans2008testq, van2006characterizing, van2007detection}  \\ \hline
%%%%%
\textbf{Gabriele Bavota}         & 3   &  \cite{bavota2012empirical, bavota2015test, tufano2016empirical}  \\ \hline
%%%%%
\rowcolor{lightgray}
\textbf{Abdallah Qusef}          & 3   &  \cite{bavota2012empirical, bavota2015test, qusef2019exploratory}  \\ \hline
%%%%%
\textbf{David Binkley}           & 3   &  \cite{bavota2012empirical, bavota2015test, qusef2019exploratory}  \\ \hline
%%%%%
\rowcolor{lightgray}
\textbf{Bart Du Bois}            & 2   &  \cite{van2006characterizing, van2007detection}  \\ \hline
%%%%%
\textbf{Serge Demeyer}           & 2   &  \cite{van2006characterizing, van2007detection}  \\ \hline
%%%%%
\rowcolor{lightgray}
\textbf{Michaela Greiler}        & 2   &  \cite{greiler2013automated, greiler2013strategies}  \\ \hline
%%%%%
\textbf{Arie Van Deursen}        & 2   &  \cite{greiler2013automated, greiler2013strategies}  \\ \hline
%%%%%
\rowcolor{lightgray}
\textbf{Margaret-Anne Storey}    & 2   &  \cite{greiler2013automated, greiler2013strategies}  \\ \hline
%%%%%
\textbf{Davide Spadini}          & 2   &  \cite{spadini2018relation, schvarcbacher2019investigating}  \\ \hline
%%%%%
\rowcolor{lightgray}
\textbf{Magiel Bruntink}         & 2   &  \cite{spadini2018relation, schvarcbacher2019investigating}  \\ \hline
%%%%%
\textbf{Jonas De Bleser}         & 2   &  \cite{de2019assessing, de2019socrates}  \\ \hline
%%%%%
\rowcolor{lightgray}
\textbf{Coen De Roover}          & 2   &  \cite{de2019assessing, de2019socrates}  \\ \hline
%%%%%
\end{tabular}
}
% \end{adjustbox}
\caption{Examples .}
\label{tab:AuthorsTable}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Tables/Metrics_Table.tex <==
\begin{table}[h!]
\caption{Metrics used in the tools.}
\vspace{-0.3cm}
\begin{adjustbox}{width=0.5\textwidth,center}
% \resizebox{\textwidth}{!}{%
% \begin{tabular*} {\textwidth}{@{\extracolsep{\stretch{1}}}*{7}{l}@{}}
\begin{tabular} {|c|l|l|l|}\hline

\rowcolor{gray!60}
\multicolumn{1}{|c}{\textbf{Tool Name}} & 
\multicolumn{1}{c}{\textbf{Metrics}} & 
\multicolumn{1}{c|}{\textbf{Target Smell Type}} \\ \hline                    

\cellcolor{gray!60} &  \# of invoked framework asserts & Assertionless \\ \cline{2-3}
%%%%%

\cellcolor{gray!60} &  \cellcolor{gray!20} \# of descriptionless asserts & \cellcolor{gray!20} Duplicated code \\ \cline{2-3}
%%%%%

\cellcolor{gray!60} &  Length of method invocations and accesses & Assertion Roulette \\ \cline{2-3}
%%%%%

\cellcolor{gray!60} &  \cellcolor{gray!20} \# of invoked production methods & \cellcolor{gray!20} Eager Test \\ \cline{2-3}
%%%%%

\cellcolor{gray!60} &  \# of invocations and accesses & Empty Test \\ \cline{2-3}
%%%%%

\cellcolor{gray!60} &  \cellcolor{gray!20} Tagging the production methods that & \cellcolor{gray!20} For Testers Only\\ 
\cellcolor{gray!60} &  \cellcolor{gray!20} are only called by test code & \cellcolor{gray!20}  \\ 
\cline{2-3}
%%%%%

\cellcolor{gray!60} & The Number of OBject Uses in setup (NOBU) & \\ 
\textbf{TestQ} \cite{breugelmans2008testq} \cellcolor{gray!60} &  Number of Fixture OBjects (NFOB) &  General Fixture \\ 
\cellcolor{gray!60} &  Average FIxture Usage &   \\ 
\cline{2-3}
%%%%%

\cellcolor{gray!60} &  \cellcolor{gray!20} \# of decision points & \cellcolor{gray!20} Indented Test \\ \cline{2-3}
%%%%%

\cellcolor{gray!60} &  \# of the number of production types &  Indirect Test \\ \cline{2-3}
%%%%%

\cellcolor{gray!60} &  \cellcolor{gray!20} Marking test commands that use & \cellcolor{gray!20} Mystery Guest \\ 
\cellcolor{gray!60} &  \cellcolor{gray!20} resource libraries (such as I/O) & \cellcolor{gray!20}  \\
\cline{2-3}
%%%%%

\cellcolor{gray!60} &  tests that invoke a toString method are tagged & Sensitive Equality \\ \cline{2-3}
%%%%%

\cellcolor{gray!60} &  \cellcolor{gray!20} Source lines of code (SLOC) & \cellcolor{gray!20} Verbose Test \\ \hline

%%%%%%%%%%%%%%%%% second Tool %%%%%%%%%%%%%%%%% 
\cellcolor{gray!60} &  UsedSetupFlds/setupFlds - deadFlds <= 0.7 & General Fixture \\ \cline{2-3}

\cellcolor{gray!60} &  \cellcolor{gray!20} usedSetupFlds = 0 AND setupFlds >=1 & \cellcolor{gray!20} Test Maverick \\ \cline{2-3}

\textbf{TestHound} \cite{greiler2013automated} \cellcolor{gray!60} &  Lack of Cohesion of test methods (LCOTM) >= 0.4 & LCOMT \\ \cline{2-3}

 \& \cellcolor{gray!60} &  \cellcolor{gray!20} |deadFlds| >= 1 & \cellcolor{gray!20} Dead Field \\ \cline{2-3}
 
\textbf{TestEvoHound} \cite{greiler2013strategies} \cellcolor{gray!60} &  |headerInit| >= 1 & Vague Header Setup \\ \cline{2-3}

\cellcolor{gray!60} &  \cellcolor{gray!20} |localVars| >= 10 & \cellcolor{gray!20} Obscure In-line setup \\ \hline
%%%%%

\end{tabular}
% \end{tabular*}

% }
\end{adjustbox}

\label{tab:Metrics_Table}
\vspace{-0.5cm}
\end{table}

==> Tables/ProjectTypeBased_Tables.tex <==
\begin{table*}
\centering
\caption{Distribution of Test Smells Per Programming Languages.
}\anthony{TODO: update with smells from new tools}

%\resizebox{\columnwidth}{!}{%
\begin{adjustbox}{width=1.0\textwidth,center}
\begin{threeparttable}
\begin{tabular} {|c|lll|c|c|}\hline

\rowcolor{gray!60}
\textbf{Programming Language} & \multicolumn{3}{c|}{\textbf{Supported Test Smell Types}}  & \textbf{Literature Usage} \\ \hline

	                & (01) Eager Test (ET)                   & (13) Constructor Initialization (CI)      & (25) Unknown Test (UT)          & \\ 
                    & (02) General Fixture (GF)              & (14) Redundant Assertion (RA)             &  (26) Duplicate Assert (DA)     & \\ 
                 	& (03) Mystery Guest (MG)                & (15) Sleepy Test (ST)                     & (27) Assertionless (AL)         & \\ 
                    & (04) Sensitive Equality (SE)           & (16) Empty Test (EmT)                     & (28) Brittle Assertion (BA)     & \\ 
\textbf{Java-Based} & (05) Assertion Roulette (AR)           & (17) Verbose Test (VT)                    & (29) Unused Input (UI)          & \cite{baker2006trex, Zeiss2006TTCN, Werner2007TTCN, Helmut2007TRex, Neukirchen2008TTCN, koochakzadeh2010tester, koochakzadeh2010tecrevis, bavota2012empirical, greiler2013automated, greiler2013strategies}  \\ 
                    & (06) Indirect Test (IT)                & (18) Test Maverick (TM)\textsuperscript{$\star$}                 & (30) Indented Test(InT)              & \cite{zhang2014empirically, huo2014improving, bavota2015test, gyori2015reliable, bell2015efficient, palomba2016diffusion, tahir2016empirical, tufano2016empirical, Palomba2017ICSME, palomba2018automatic}\\ 
                    & (07) Resource Optimism (RO)            & (19) Dead Field (DF)\textsuperscript{$\star$}                    & (31) Dependent Test (DepT)           & \cite{Spadini2018ICSME, gambi2018practical, virginio2019influence, peruma2019CASCON, qusef2019exploratory, palomba2019smell, grano2019scented, biagiola2019web, schvarcbacher2019investigating, Grano2019TSE}\\ 
                    & (08) Lazy Test (LT)                    & (20) Obscure In-line Setup Smell(OISS)\textsuperscript{$\star$}  & (32) Default Test (DT)               & \cite{Spadini2020MSR, peruma2020FSE, lambiase2020just, virginio2020empirical, virginio2020jnose, Santana2020SBES, Panichella2020ICSME, Soares2020SAST, Kim2020ICSE, Pecorelli2020AVI}\\ 
                    & (09) For Testers Only (FTO)            & (21) Vague Header Setup(VHS)\textsuperscript{$\star$}            & (33) Ignored Test (IgT)              & \cite{Biagiola2020ICST, Fraser2020ICSTW, Peruma2020IWoR, Martinez2020ICSE}\\ 
                    & (10) Duplicated Code (DC)              & (22) Exception Handling (EH)                                     & (34) Fire and Forget (FF)            & \\
                    & (11) Conditional Test Logic (CTL)      & (23) Magic Number Test (MNT)                                     & (35) Test Run War(TRW)               &  \\ 
                    & (12) Lack of Cohesion of Test Methods (LCM)\textsuperscript{$\star$}                                      & (24) Redundant Print (RP)            &           &  \\ \hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
\rowcolor{gray!30}                      
\textbf{Scala-Based}     & (01) Assertion Roulette (AR)           & (03) Exception Handling (EH)  & (05) Sensitive Equality (SE) & \cite{de2019socrates,de2019assessing} \\ 
\rowcolor{gray!30}
                         & (02) Eager Test (ET)                   & (04) Mystery Guest (MG)                 & (06) General Fixture (GF)    & \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%                         
                         & (01) Overreferencing (OF)                   & (10) Unclassied MethodCategory (UMC)                  & (19) Unusual Test Order (UTO)       &  \\  
                         & (02) Assertionless Test (AL)                & (11) Unused Shared-Fixture Variables (USFV)           & (20) Teardown Only Test (TOT)       &  \\ 
                         & (03) Proper Organization (PO)               & (12) Early Returning Test (ERT)                       & (21) Test-Class Name (TCN)          &  \\ 
                         & (04) Overcommented Test (OCT)               & (13) Max Instance Variables (MIV)                     & (22) Empty Shared-Fixture (ESF)     &  \\ 
\textbf{SmallTalk-Based} & (05) Anonymous Test (AT)                    & (14) Under-the-carpet Assertion (UCA)                 & (23) Transcripting Test (TT)        & \cite{reichhart2007rule, Delplanque2019ICSE} \\ 
                         & (06) Long Test (LoT)                        & (15) Empty Test-MethodCategory (ETMC)                 & (24) Empty MethodCategory (EMC)     &  \\ 
                         & (07) Mixed Selectors (MS)                   & (16) Test-MethodCategory Name (TMC)                   & (25) Returning Assertion (RA)       &  \\ 
                         & (08) Control Logic (ConL)                   & (17) Under-the-carpet failing Assertion (UCFA)        & (26) Comments Only Test (COT)       &  \\  
                         & (09) Abnormal UTF-Use (AUU)                 & (18) Likely ineffective Object-Comparison (LIOC)      & (27) Guarded Test (GT)              &  \\ \hline
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%                         
\rowcolor{gray!30}                          & (01) Assertionless Test (AL)                & (05) Empty Test (EmT)                                 &  (09) Indirect Test (IT)            &  \\ 
\rowcolor{gray!30} \textbf{C++-Based}       & (02) Assertion Roulette (AR)                & (06) For Testers Only (FTO)                           &  (10) Mystery Guest (MG)            &  \cite{breugelmans2008testq}\\ 
 \rowcolor{gray!30}                         & (03) Duplicated Code (DC)                   & (07) General Fixture (GF)                             &  (11) Sensitive Equality (SE)       &  \\ 
\rowcolor{gray!30}                          & (04) Eager Test (ET)                        & (08) Indented Test(InT)                               &  (12) Verbose Test (VT)             &  \\ \hline

 

\end{tabular}
\begin{tablenotes}
            \item $\star\,$ These smells derived from Test fixture smells based on \cite{greiler2013automated}.
        \end{tablenotes}
\end{threeparttable}
\end{adjustbox}
% {\raggedright \textbf{Note:} Test Fixture (TF), Test Maverick smell, Dead Field smell, Obscure In-line Setup Smell and Vague Header Setup. \par}
        
%}

\label{tab:ProjectBased}

\end{table*}





% \cite{huo2014improving,schvarcbacher2019investigating,palomba2019smell,bavota2015test,van2006characterizing}\cite{bavota2012empirical,palomba2017does,van2007detection,grano2019scented,peruma2019distribution}\cite{virginio2019influence,palomba2016diffusion,greiler2013strategies,greiler2013automated,qusef2019exploratory}\cite{spadini2018relation,tahir2016empirical,tufano2016empirical,palomba2018automatic} \anthony{Wajdi -- why do you have four citation groups?} \\ 

==> Tables/TestSmellDefinition.tex <==

\begin{table*}
\centering
\caption{Test smells definition.}\anthony{Table needs to be sorted alphabetically based the test smell name}

% \resizebox{\columnwidth}{!}{%
\begin{adjustbox}{width=1.1\textwidth,center}
\begin{threeparttable}
\begin{tabular} {|c|l|l|l|c|}\hline
\rowcolor{gray!60}
\textbf{No} & \textbf{Test Smell Type} & \textbf{Abbr} & \textbf{Definition} & \textbf{Ref} \\ \hline   

\textbf{1} & \textbf{Eager Test} & \textbf{ET} &  A method that call several methods of object to be tested.   & \cite{van2001refactoring, bavota2012empirical, peruma2020FSE} \\ \hline
%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\textbf{2} & \textbf{General Fixture} & \textbf{GF} &  This smell emerge when
{\fontfamily{qcr}\selectfont setUp()}
fixture is too general, and the test method only access part of it.   & \cite{van2001refactoring, bavota2012empirical, peruma2020FSE} \\ \hline
%%%%%%%%%%%%%%%

\textbf{3} & \textbf{Mystery Guest} & \textbf{MG} &    A test that uses an external resources, such as database that containing test data. & \cite{van2001refactoring, bavota2012empirical, peruma2020FSE} \\ \hline  
%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\textbf{4} & \textbf{Sensitive Equality} & \textbf{SE} &  Occurs  when an assertion have equality check by using toString method.  & \cite{van2001refactoring, bavota2012empirical, peruma2020FSE} \\ \hline
%%%%%%%%%%%%%%%
\textbf{5} & \textbf{Assertion Roulette} & \textbf{AR} &  Occurs when a test method that having more than one assertion and no explanation for each one.    & \cite{van2001refactoring, bavota2012empirical, peruma2020FSE} \\ \hline
%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\textbf{6} & \textbf{Indirect Testing} & \textbf{IT} &   A test that interacts to a corresponding class by using another class.   & \cite{van2001refactoring, bavota2012empirical} \\ \hline
%%%%%%%%%%%%%%%
\textbf{7} & \textbf{Resource Optimism} & \textbf{RO} &  A test that make an assumption about the existence of external resources such as file.    & \cite{van2001refactoring, bavota2012empirical, peruma2020FSE} \\ \hline
%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\textbf{8} & \textbf{Lazy Test } & \textbf{LT} &  Occurs when multiple test methods check the same method of production object.  & \cite{van2001refactoring, bavota2012empirical, peruma2020FSE} \\ \hline
%%%%%%%%%%%%%%%
\textbf{9} & \textbf{For Testers Only} & \textbf{FTO} &  A production class that contain methods that only used for test method.  & \cite{van2001refactoring, bavota2012empirical} \\ \hline
%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\textbf{10} & \textbf{Duplicated code} & \textbf{DC} &  A test method that have redundancy in the code that is unnecessary.  & \cite{van2001refactoring, bavota2012empirical} \\ \hline
%%%%%%%%%%%%%%%
\textbf{11} & \textbf{Conditional Test Logic} & \textbf{CTL} & A test method that contain a conditional statement as a prerequisite to execute test statement.   & \cite{peruma2020FSE} \\ \hline
%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\textbf{12} & \textbf{Lack of Cohesion of Methods} & \textbf{LCM} &  When test method are grouped together in one test class but they are not cohesive. & \cite{greiler2013automated, greiler2013strategies, palomba2018automatic} \\ \hline
%%%%%%%%%%%%%%%
\textbf{13} & \textbf{Constructor Initialization} & \textbf{CI} &   A test class that contain a constructor.  & \cite{peruma2020FSE} \\ \hline
%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\textbf{14} & \textbf{Redundant Assertion} & \textbf{RA} &  A test method that have an assertion statements that is permanently true or false.  & \cite{peruma2020FSE} \\ \hline
%%%%%%%%%%%%%%%
\textbf{15} & \textbf{Sleepy Test} & \textbf{ST} &  Occurs when a test method have an explicit wait.  & \cite{peruma2020FSE} \\ \hline
%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\textbf{16} & \textbf{Empty Test} & \textbf{EmT} &  A test method that is empty or dose not have an executable statements.  & \cite{peruma2020FSE} \\ \hline
%%%%%%%%%%%%%%%
\textbf{17} & \textbf{Verbose Test} & \textbf{VT} &   A test code that is complex and not simple or clean. & \cite{JNose2019, TestQ2008} \\ \hline
%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\textbf{} & \textbf{} & \textbf{} & Exist when a test class has a test method with implicit setup, however, the test methods is independent &  \\ 
\rowcolor{gray!30}
\textbf{18} & \textbf{Test Maverick} & \textbf{TM} & from that setup. & \cite{greiler2013automated, greiler2013strategies} \\ 
\hline
%%%%%%%%%%%%%%%
\textbf{19} & \textbf{Dead Field} & \textbf{DF} &  When a class have a field that never used by any test methods.   & \cite{greiler2013automated, greiler2013strategies} \\ \hline
%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\textbf{20} & \textbf{Obscure In-line Setup Smell} & \textbf{OISS} &  A test that have too much setup functionality in the test method.  & \cite{greiler2013automated, greiler2013strategies}  \\ \hline
%%%%%%%%%%%%%%%
\textbf{21} & \textbf{Vague Header Setup} & \textbf{VHS} &  A field that is initialized in class header but not explicitly defined in code.    & \cite{greiler2013automated, greiler2013strategies} \\ \hline
%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\textbf{22} & \textbf{Exception Heandling} & \textbf{EH} &  Occurs when the use of custom exception handling code instead of using JUnit's exception handling feature.   & \cite{peruma2020FSE} \\ \hline
%%%%%%%%%%%%%%%
\textbf{23} & \textbf{Magic Number Test} & \textbf{MNT} &   A test method that contain undocumented numerical values.    & \cite{peruma2020FSE} \\ \hline
%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\textbf{24} & \textbf{Redundant Print} & \textbf{RP} &   A test method that have print statement.    & \cite{peruma2020FSE} \\ \hline
%%%%%%%%%%%%%%%
\textbf{25} & \textbf{Unknown Test} & \textbf{UT} &  A test method without an assertion statement and non-descriptive name.     & \cite{peruma2020FSE} \\ \hline
%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\textbf{26} & \textbf{Duplicate Assert} & \textbf{DA} &   Occurs when a test method have the exact assertion multiple time with in the same test method.    & \cite{peruma2020FSE} \\ \hline
%%%%%%%%%%%%%%%
\textbf{27} & \textbf{Assertionless}\tnote{*} & \textbf{AL} &   A test that is acting to assert data and functionality, but does not.    & \cite{peruma2020FSE, virginio2019influence, TestQ2008} \\ \hline
%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\textbf{28} & \textbf{Brittle Assertion} & \textbf{BA} &  A test method that have an a assertions that check data input.     & \cite{huo2014improving} \\ \hline
%%%%%%%%%%%%%%%
\textbf{29} & \textbf{Unused Input} & \textbf{UI} &   An inputs that are control by the test.    & \cite{huo2014improving} \\ \hline
%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\textbf{30} & \textbf{Indented Test} & \textbf{InT} &  A test that contain a large number of decision points, too much use of loop and conditional statements.    & \cite{TestQ2008} \\ \hline
%%%%%%%%%%%%%%%
\textbf{31} & \textbf{Dependent Test} & \textbf{DepT} &  A test that only execute on the  dependency of successful execution of other test.      & \cite{virginio2019influence} \\ \hline
%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\textbf{32} & \textbf{Default Test} & \textbf{DT} &   A test that have classes that are created by default.      & \cite{peruma2020FSE} \\ \hline
%%%%%%%%%%%%%%%
\textbf{33} & \textbf{Ignored Test} & \textbf{IgT} &   A test method that uses an ignore annotation which will prevent the test method from running.      & \cite{peruma2020FSE} \\ \hline
%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\textbf{34} & \textbf{Fire and Forget} & \textbf{FF} &  A test that is exiting prematurely  without waiting for the results of external calls.      & \cite{palomba2019smell} \\ \hline
%%%%%%%%%%%%%%%
\textbf{35} & \textbf{Test Run War} & \textbf{TRW} &   A test that fail when more than one programmer run them.      & \cite{van2001refactoring, bavota2012empirical} \\ \hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%% samlltalk smells %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\textbf{36} & \textbf{Overreferencing} & \textbf{OF} &  A test that causes duplication by creating unnecessary dependencies.       & \cite{reichhart2007rule} \\ \hline
%%%%%%
\textbf{37} & \textbf{Proper Organization} & \textbf{PO} &  A test method that violates a test conventions.     & \cite{reichhart2007rule} \\ \hline
%%%%%%

\rowcolor{gray!30}
\textbf{38} & \textbf{Overcommented Test} & \textbf{OCT} &  A test with a numerous test comments.      & \cite{reichhart2007rule} \\ \hline
%%%%%%
\textbf{39} & \textbf{Anonymous Test} & \textbf{AT} &   A test method with a meaningless, unclear method name.      & \cite{reichhart2007rule} \\ \hline
%%%%%%
\rowcolor{gray!30}
\textbf{40} & \textbf{Long Test} & \textbf{LoT} & A test with many LOCs/statments.       & \cite{reichhart2007rule} \\ \hline
%%%%%%
\textbf{41} & \textbf{Mixed Selectors} & \textbf{MS} & Violates test conventions by confusing between testing and non-testing methods.  & \cite{reichhart2007rule}   \\ \hline
%%%%%%
\rowcolor{gray!30}
\textbf{42} & \textbf{Control Logic} & \textbf{ConL} & A test method that controls test data flow by methods such as debug or halt. & \cite{reichhart2007rule} \\ \hline
%%%%%%
\textbf{43} & \textbf{Abnormal UTF-Use} & \textbf{AUU} & Overriding the  default behavior of the testing framework by test-suite.   & \cite{reichhart2007rule} \\ \hline
%%%%%%
\rowcolor{gray!30}
\textbf{44} & \textbf{Unclassified MethodCategory} & \textbf{UMC} &  A test method that is not organized by a method category.  & \cite{reichhart2007rule} \\ \hline
%%%%%%
\textbf{45} & \textbf{Unused Shared-Fixture Variables} & \textbf{USFV} &  It occurs when a piece of the fixture are never used.  & \cite{reichhart2007rule}  \\ \hline
%%%%%%
\rowcolor{gray!30}
\textbf{46} & \textbf{Early Returning Test} & \textbf{ERT} & A test method that return a value too early which may drop assertions. & \cite{reichhart2007rule} \\ \hline
%%%%%%
\textbf{47} & \textbf{Max Instance Variables} & \textbf{MIV} &  A test method that has a large number of fixture.  & \cite{reichhart2007rule} \\ \hline
%%%%%%
\rowcolor{gray!30}
\textbf{48} & \textbf{Under-the-carpet failing Assertion} & \textbf{UCFA} &  A test method that have a failing assertion statement that puts into comment.   & \cite{reichhart2007rule} \\ \hline
%%%%%%
\textbf{49} & \textbf{Empty Test-MethodCategory} & \textbf{ETMC} &  A test method with empty test method category.   & \cite{reichhart2007rule} \\ \hline
%%%%%%
\rowcolor{gray!30}
\textbf{50} & \textbf{Test-MethodCategory Name} & \textbf{TMC} &  A test method have a meaningless name.   & \cite{reichhart2007rule} \\ \hline
%%%%%%
\textbf{51} & \textbf{Under-the-carpet Assertion} & \textbf{UCA} &  A test that have an assertions that are put in a comment.   & \cite{reichhart2007rule} \\ \hline
%%%%%%
\rowcolor{gray!30}
\textbf{52} & \textbf{Likely ineffective Object-Comparison} & \textbf{LIOC} & A test that compare between objects that will never fail.    & \cite{reichhart2007rule} \\ \hline
%%%%%%
\textbf{53} & \textbf{Unusual Test Order} & \textbf{UTO} &   A test that is calling other test explicitly.  & \cite{reichhart2007rule} \\ \hline
%%%%%%
\rowcolor{gray!30}
\textbf{54} & \textbf{Teardown Only Test} & \textbf{TOT} &  It exists when a test-suite only specifying teardown.   & \cite{reichhart2007rule} \\ \hline
%%%%%%
\textbf{55} & \textbf{Test-Class Name} & \textbf{TCN} &  A test that have a class with meaningless name.   & \cite{reichhart2007rule} \\ \hline
%%%%%%
\rowcolor{gray!30}
\textbf{56} & \textbf{Empty Shared-Fixture} & \textbf{ESF} &   A test that define a fixture with empty body.  & \cite{reichhart2007rule} \\ \hline
%%%%%%
\textbf{57} & \textbf{Transcripting Test} & \textbf{TT} &  A test that is printing and logging to the console. & \cite{reichhart2007rule} \\ \hline
%%%%%%
\rowcolor{gray!30}
\textbf{58} & \textbf{Empty MethodCategory} & \textbf{EMC} &  A test method with empty method category.  & \cite{reichhart2007rule} \\ \hline
%%%%%%
\textbf{59} & \textbf{Returning Assertion} & \textbf{RA} &  A test method that have an assertion that is returning values to the method. & \cite{reichhart2007rule} \\ \hline
%%%%%%
\rowcolor{gray!30}
\textbf{60} & \textbf{Comments Only Test} & \textbf{COT} &   A test that has been put into a comments.  & \cite{reichhart2007rule} \\ \hline
%%%%%%
\textbf{61} & \textbf{Guarded Test} & \textbf{GT} &  A test that have conditional branches like ifTrue:aCode or ifFalse:aCode.  & \cite{reichhart2007rule} \\ \hline
%%%%%%
% \textbf{62} & \textbf{Test Clones}  & \textbf{TC} & & \cite{} \\ \hline
%%%%%%
\rowcolor{gray!30}
\textbf{62} & \textcolor{red}{ \textbf{Test Redundancy}}  & \textbf{TR} &  0000& \cite{koochakzadeh2010tecrevis, koochakzadeh2010tester} \\ \hline
%%%%%%  
\textbf{63} & \textcolor{red}{ \textbf{TTCN-3**}}  & \textbf{TTCN} &  0000& \cite{baker2006trex} \\ \hline





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\end{tabular}

\begin{tablenotes}
            \item The test smells from (36) - (60) are related to SamllTalk.
            \item[*] This test smell occurs in  SmallTalk \& Java with having same purpose and definition.
            \item[**] This test smell occurs in TRex tool, and the exact smell types are not listed in the paper.
        \end{tablenotes}
        
\end{threeparttable}

\end{adjustbox}
% }

\label{tab:Test_Definitions}
\end{table*}




==> Tables/TestSmellTypes.tex <==
\begin{table*}
\centering
% \resizebox{\columnwidth}{!}{%
\begin{adjustbox}{width=1.1\textwidth,center}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}\hline
\rowcolor{gray!60}
\textbf{Study} & \textbf{ET} & \textbf{GF} & \textbf{MG} & \textbf{SE} & \textbf{AR} & \textbf{IT} & \textbf{RO} & \textbf{LT} & \textbf{FTO} & \textbf{DC} & \textbf{CTL} & \textbf{LCM} & \textbf{CI} & \textbf{RA} & \textbf{ST} & \textbf{EmT} & \textbf{VT} & \textbf{TM} & \textbf{DF} & \textbf{OLS} & \textbf{VHS} & \textbf{DT} & \textbf{EH} & \textbf{IgT} & \textbf{MNT} & \textbf{RP} & \textbf{UT} & \textbf{DA} & \textbf{AL} & \textbf{LF} & \textbf{BF} & \textbf{BA} & \textbf{UI} & \textbf{InT} & \textbf{DepT} & \textbf{FF} & \textbf{TRW} & \textbf{Total}\\  \hline   

\cite{virginio2019influence} & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ &  &  & $\surd$ & & $\surd$
& $\surd$ & $\surd$  & $\surd$ & $\surd$ & & & & & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ & $\surd$  &  $\surd$ 
& $\surd$  &  & & & & & $\surd$ & & & \textbf{21} \\ \hline 
%%%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\cite{peruma2019distribution} & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ &  &  & $\surd$ & & $\surd$
& $\surd$ & $\surd$  & $\surd$ &  & & & & & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ & $\surd$  &  $\surd$ 
& $\surd$  &  & & & & &  & & & \textbf{19} \\ \hline 
%%%%%%%%%%%%%%%%%
\cite{breugelmans2008testq} & $\surd$ &  $\surd$ & $\surd$  & $\surd$ & $\surd$ & $\surd$ &   &   & $\surd$ & $\surd$ &   & &  
&  &    & $\surd$ & $\surd$ & & & & &   &   &  &   &   &    &    
& $\surd$ &  & & & & $\surd$ &  & & & \textbf{12} \\ \hline 
%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\cite{bavota2012empirical} & $\surd$ &  $\surd$ & $\surd$  & $\surd$ & $\surd$ & $\surd$ &   & $\surd$  & $\surd$ & $\surd$ &   & &  
&  &    &  &  & & & & &   &   &  &   &   &    &    
&  &  & & & &  &  & & & \textbf{9} \\ \hline 
%%%%%%%%%%%%%%%%% 
\cite{bavota2015test} & $\surd$ &  $\surd$ & $\surd$  & $\surd$ & $\surd$ & $\surd$ &   & $\surd$  & $\surd$ & $\surd$ &   & &  
&  &    &  &  & & & & &   &   &  &   &   &    &    
&  &  & & & &  &  & & & \textbf{9} \\ \hline 
%%%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\cite{tahir2016empirical} & $\surd$ &  $\surd$ & $\surd$  & $\surd$ & $\surd$ & $\surd$ &   & $\surd$  &  & $\surd$ &   & & 
&  &    &  &  & & & & &   &   &  &   &   &    &    
&  & $\surd$ & & & &  &  & & & \textbf{9} \\ \hline 
%%%%%%%%%%%%%%%%%
\cite{schvarcbacher2019investigating} & $\surd$ &  & $\surd$ & $\surd$ &  &  & $\surd$ &   &  &  & $\surd$ & & $\surd$
& $\surd$ & $\surd$ &  & $\surd$ & & & & &   &   &  &   &   &    &    
&  &  & & & &  &  & & & \textbf{9} \\ \hline 
%%%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\cite{palomba2016diffusion} & $\surd$ &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &   & $\surd$ & $\surd$ &  & & 
&  &  &  &  & & & & &   &   &  &   &   &    &    
&  &  & & & &  &  & & & \textbf{8} \\ \hline 
%%%%%%%%%%%%%%%%%
\cite{qusef2019exploratory} & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  &  &   & $\surd$ & $\surd$ &  & & 
&  &  &  &  & & & & &   &   &  &   &   &    &    
&  &  & & & &  &  & & & \textbf{7} \\ \hline 
%%%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\cite{grano2019scented} & $\surd$ &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &   & $\surd$ &  &  & & 
&  &  &  &  & & & & &   &   &  &   &   &    &    
&  &  & & & &  &  & & & \textbf{7} \\ \hline 
%%%%%%%%%%%%%%%%%
\cite{greiler2013automated} &  & $\surd$ &  &  &  &  &  &   &  &  &  & $\surd$ & 
&  &  &  &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  &   &  &   &   &    &    
&  &  & & & &  &  & & & \textbf{6} \\ \hline 
%%%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\cite{spadini2018relation} &  & $\surd$ &  &  &  &  &  &   &  &  &  & $\surd$ & 
&  &  &  &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  &   &  &   &   &    &    
&  &  & & & &  &  & & & \textbf{6} \\ \hline 
%%%%%%%%%%%%%%%%%
\cite{de2019assessing} & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  &  & $\surd$  &  &  &  &  & 
&  &  &  &  &  &  &  &  &  &   &  &   &   &    &    
&  &  & & & &  &  & & & \textbf{6} \\ \hline 
%%%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\cite{de2019socrates} & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  &  & $\surd$  &  &  &  &  & 
&  &  &  &  &  &  &  &  &  &   &  &   &   &    &    
&  &  & & & &  &  & & & \textbf{6} \\ \hline 
%%%%%%%%%%%%%%%%%
\cite{tufano2016empirical} & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  &  &   &  &  &  &  & 
&  &  &  &  &  &  &  &  &  &   &  &   &   &    &    
&  &  & & & &  &  & & & \textbf{5} \\ \hline 
%%%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\cite{palomba2019smell} &  &  &  &  &  & $\surd$ & $\surd$ &   &  &  & $\surd$ &  & 
&  &  &  &  &  &  &  &  &  &   &  &   &   &    &    
&  &  & & & &  &  & $\surd$ & $\surd$ & \textbf{5} \\ \hline
%%%%%%%%%%%%%%%%%
\cite{van2006characterizing} & $\surd$ & $\surd$ &  &  &  &  &  &   &  &  &  &  & 
&  &  &  &  &  &  &  &  &  &   &  &   &   &    &    
&  & $\surd$ & $\surd$ &  & &  &  &  &  & \textbf{4} \\ \hline 
%%%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\cite{palomba2017does} &  &  &  &  &  & $\surd$ & $\surd$ &   &  &  &  &  & 
&  &  &  &  &  &  &  &  &  &   &  &   &   &    &    
&  &  &  &  & &  &  &  & $\surd$ & \textbf{3} \\ \hline 
%%%%%%%%%%%%%%%%%   
\cite{palomba2018automatic} & $\surd$ & $\surd$ &  &  &  &  &  &   &  &  &  & $\surd$ & 
&  &  &  &  &  &  &  &  &  &   &  &   &   &    &    
&  &  &  &  & &  &  &  &  & \textbf{3} \\ \hline 
%%%%%%%%%%%%%%%%% 
\rowcolor{gray!30}
\cite{van2007detection} & $\surd$ & $\surd$ &  &  &  &  &  &   &  &  &  &  & 
&  &  &  &  &  &  &  &  &  &   &  &   &   &    &    
&  &  &  &  & &  &  &  &  & \textbf{2} \\ \hline 
%%%%%%%%%%%%%%%%%   
\cite{huo2014improving} &  &  &  &  &  &  &  &   &  &  &  &  & 
&  &  &  &  &  &  &  &  &  &   &  &   &   &    &    
&  &  &  & $\surd$ & $\surd$ &  &  &  &  & \textbf{2} \\ \hline 
\end{tabular}
\end{adjustbox}
% }
\caption{ Distribution  of  .}
\label{tab:AllNo}
\end{table*}














% \begin{table*}
% \centering
% % \resizebox{\columnwidth}{!}{%
% \begin{adjustbox}{width=1.1\textwidth,center}
% \begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}\hline

% \textbf{Study} & \textbf{MG} & \textbf{RO} & \textbf{ET} & \textbf{AR} & \textbf{IT} & \textbf{FTO} & \textbf{SE} & \textbf{DA} & \textbf{GF} & \textbf{MG} & \textbf{LT} & \textbf{CTL} & \textbf{CI} & \textbf{DT} & \textbf{DepT} & \textbf{EpT} & \textbf{ECT} & \textbf{IgT} & \textbf{MNT} & \textbf{RP} & \textbf{RA} & \textbf{ST} & \textbf{UT} & \textbf{VT} & \textbf{TRW} & \textbf{FF} & \textbf{DC} & \textbf{AL} & \textbf{InT} & \textbf{LCM} & \textbf{} & \textbf{} & \textbf{Total}\\  \hline   

% \cite{breugelmans2008testq} & &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & & $\surd$ & $\surd$ & & & & & $\surd$ & & & & & & & & & $\surd$ & & & $\surd$ & $\surd$ & $\surd$ & & & & \textbf{12} \\ \hline 

% \cite{palomba2018automatic} & & & $\surd$ & & & & & & $\surd$ &  & & & & & & & & & & & & & & & & & & & & $\surd$ & && \textbf{3} \\ \hline 

% \cite{tufano2016empirical} & $\surd$ & & $\surd$ & $\surd$ & & & $\surd$ & & $\surd$ &  & & & & & & & & & & & & & & & & & & & & & && \textbf{5} \\ \hline 

% \cite{tahir2016empirical} &  &  & $\surd$ & $\surd$ & $\surd$ & & $\surd$ & & $\surd$ & $\surd$ & $\surd$ & & & & & & & & & & & & & & & & $\surd$ & $\surd$ & & &  & & \textbf{9} \\ \hline 

% \cite{spadini2018relation} &  & $\surd$ & $\surd$ & $\surd$ & & & $\surd$ & &  & $\surd$ & $\surd$ & & & & & & & & & & & & & & & & & & & & && \textbf{6} \\ \hline 

% \cite{qusef2019exploratory} &  &  & $\surd$ & $\surd$ & & $\surd$ & $\surd$ & & $\surd$ & $\surd$ &  & & & & & & & & & & & & & & & & $\surd$ & & & & & & \textbf{7} \\ \hline 

% \cite{palomba2016diffusion} &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & &  & $\surd$ &  & & & & & & & & & & & & & & & & $\surd$ & & & & & & \textbf{8} \\ \hline 

% % review the below
% \cite{virginio2019influence} &  & $\surd$ &  & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  &  &  & & & & & & \textbf{20} \\ \hline 

% % the reset of papers

% \cite{peruma2019distribution} &  & $\surd$ &  & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  &  &  & & & & & & \textbf{20} \\ \hline 

% \cite{virginio2019influence} &  & $\surd$ &  & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  &  &  & & & & & & \textbf{20} \\ \hline 

% \cite{virginio2019influence} &  & $\surd$ &  & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  &  &  & & & & & & \textbf{20} \\ \hline 

% \cite{virginio2019influence} &  & $\surd$ &  & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  &  &  & & & & & & \textbf{20} \\ \hline 

% \cite{virginio2019influence} &  & $\surd$ &  & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  &  &  & & & & & & \textbf{20} \\ \hline 

% \cite{virginio2019influence} &  & $\surd$ &  & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  &  &  & & & & & & \textbf{20} \\ \hline 

% \cite{virginio2019influence} &  & $\surd$ &  & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  &  &  & & & & & & \textbf{20} \\ \hline 

% \cite{virginio2019influence} &  & $\surd$ &  & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  &  &  & & & & & & \textbf{20} \\ \hline 

% \cite{virginio2019influence} &  & $\surd$ &  & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  &  &  & & & & & & \textbf{20} \\ \hline 
% \end{tabular}
% \end{adjustbox}
% % }
% \caption{ Distribution  of  .}
% \label{tab:AllNo}
% \end{table*}




==> Tables/TestSmellTypesByTools.tex <==
\begin{table*}
\centering
\caption{Distribution of the number of the test smells detected by Tools}

% \resizebox{\columnwidth}{!}{%
\begin{adjustbox}{width=1.1\textwidth,center}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}\hline
\rowcolor{gray!60}
\textbf{Study} & \textbf{ET} & \textbf{GF} & \textbf{MG} & \textbf{SE} & \textbf{AR} & \textbf{IT} & \textbf{RO} & \textbf{LT} & \textbf{FTO} & \textbf{DC} & \textbf{CTL} & \textbf{LCM} & \textbf{CI} & \textbf{RA} & \textbf{ST} & \textbf{EmT} & \textbf{VT} & \textbf{TM} & \textbf{DF} & \textbf{OISS} & \textbf{VHS} & \textbf{DT} & \textbf{EH} & \textbf{MNT} & \textbf{RP} & \textbf{UT} & \textbf{DA} & \textbf{AL} & \textbf{BA} & \textbf{UI} & \textbf{InT} & \textbf{DepT}  & \textbf{\textit{Total}}\\  \hline   

\textbf{JNose} \cite{virginio2019influence} & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ &  &  & $\surd$ & & $\surd$
& $\surd$ & $\surd$  & $\surd$ & $\surd$ & & & & & $\surd$ & $\surd$  & $\surd$ & $\surd$ & $\surd$  &  $\surd$ 
& $\surd$  & & & & $\surd$ & \textbf{21} \\ \hline 
%%%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\textbf{\textsc{tsDetect}} \cite{peruma2019distribution} & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  & $\surd$ & $\surd$ &  &  & $\surd$ & & $\surd$
& $\surd$ & $\surd$  & $\surd$ &  & & & & & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$  &  $\surd$ 
& $\surd$  & & & &  & \textbf{19} \\ \hline 
%%%%%%%%%%%%%%%%%
\textbf{TestQ} \cite{breugelmans2008testq} & $\surd$ &  $\surd$ & $\surd$  & $\surd$ & $\surd$ & $\surd$ &   &   & $\surd$ & $\surd$ &   & &  
&  &    & $\surd$ & $\surd$ & & & & &   &   &   &   &    &    
& $\surd$ & & & $\surd$ &  & \textbf{12} \\ \hline 
%%%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\textbf{Unnamed} \cite{bavota2012empirical} & $\surd$ &  $\surd$ & $\surd$  & $\surd$ & $\surd$ & $\surd$ &   & $\surd$  & $\surd$ & $\surd$ &   & &  
&  &    &  &  & & & & &   &   &   &   &    &    
&  & & &  &  & \textbf{9} \\ \hline 
%%%%%%%%%%%%%%%%%
\textbf{TestHound} \cite{greiler2013automated} &  & $\surd$ &  &  &  &  &  &   &  &  &  & $\surd$ & 
&  &  &  &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  &    &   &   &    &    
&   & & &  &  & \textbf{6} \\ \hline 
%%%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\textbf{TestEvoHound} \cite{greiler2013strategies} &  & $\surd$ &  &  &  &  &  &   &  &  &  & $\surd$ & 
&  &  &  &  & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  &    &   &   &    &    
&   & & &  &  & \textbf{6} \\ \hline 
%%%%%%%%%%%%%%%%%
\textbf{SoCRATES} \cite{de2019socrates} & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  &  & $\surd$  &  &  &  &  & 
&  &  &  &  &  &  &  &  &  &    &   &   &    &    
&   & & &  &  & \textbf{6} \\ \hline 
%%%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\textbf{HistoryMiner} \cite{tufano2016empirical} & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &  &  &   &  &  &  &  & 
&  &  &  &  &  &  &  &  &  &   &   &   &    &    
&   & & &  &  & \textbf{5} \\ \hline 
%%%%%%%%%%%%%%%%%
\textbf{TASTE} \cite{palomba2018automatic} & $\surd$ & $\surd$ &  &  &  &  &  &   &  &  &  & $\surd$ & 
&  &  &  &  &  &  &  &  &  &    &   &   &    &    
&   &  & &  &  & \textbf{3} \\ \hline 
%%%%%%%%%%%%%%%%%
\rowcolor{gray!30}
\textbf{OraclePolish} \cite{huo2014improving} &  &  &  &  &  &  &  &   &  &  &  &  & 
&  &  &  &  &  &  &  &  &  &   &   &   &    &    
&  & $\surd$ & $\surd$ &  &  & \textbf{2} \\ \hline 
\textbf{\textit{Total}} &  \textbf{7} &  \textbf{9} &  \textbf{6} &  \textbf{6} &  \textbf{6} &  \textbf{2} &  \textbf{2} &  \textbf{4} &  \textbf{2} &  \textbf{2} &  \textbf{2} &  \textbf{3} &  \textbf{2}
&  \textbf{2} &  \textbf{2} &  \textbf{3} &  \textbf{2} &  \textbf{2} &  \textbf{2} &  \textbf{2} &  \textbf{2} &  \textbf{2} &   \textbf{2}  &   \textbf{2} &   \textbf{2} &   \textbf{2}  &   \textbf{2}  
&  \textbf{3}  &  \textbf{1} &  \textbf{1} &  \textbf{1}  &   \textbf{1} & -- \\ \hline 
%%%%%%%%%%%%%%%%%
\end{tabular}
\end{adjustbox}
% }
\label{tab:TestSmellTypes}
\end{table*}

==> Tables/TestSmellTypesByTools_v2.tex <==
\begin{table*}
\centering
\caption{Distribution of test smells detected by the test smell detection tools.} \anthony{TODO: update with smells from new tools}
\label{tab:TestSmellTypes_v2}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}|l|cccccccccccccccc|r|@{}}
\rowcolor{gray!60}
\textbf{Test Smell} &
  \textbf{\begin{tabular}[c]{@{}c@{}}JNose Test\\ {\cite{virginio2019influence}}\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}\textsc{tsDetect}\\ {\cite{peruma2020FSE}}\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}TestQ\\ {\cite{breugelmans2008testq}}\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Unnamed\\ {\cite{bavota2012empirical}}\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}TestHound\\ {\cite{greiler2013automated}}\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}TestEvoHound\\ {\cite{greiler2013strategies}}\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}SoCRATES\\ {\cite{de2019socrates}}\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}HistoryMiner\\ {\cite{tufano2016empirical}}\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}TASTE\\ {\cite{palomba2018automatic}}\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}OraclePolish\\ {\cite{huo2014improving}}\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}TestLint\\ {\cite{reichhart2007rule}}\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}RAIDE\\ {\cite{}}\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}DARTS\\ {\cite{}}\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}DTDetector\\ {\cite{}}\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}TeCReVis\\ {\cite{}}\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}TeReDetect\\ {\cite{}}\end{tabular}} &
%  \textbf{\begin{tabular}[c]{@{}c@{}}TRex\\ {\cite{}}\end{tabular}} &
%  \textbf{\begin{tabular}[c]{@{}c@{}}POLDET\\ {\cite{}}\end{tabular}} &
%  \textbf{\begin{tabular}[c]{@{}c@{}}TEDD\\ {\cite{}}\end{tabular}} &
%  \textbf{\begin{tabular}[c]{@{}c@{}}PRADET\\ {\cite{}}\end{tabular}} &
%  \textbf{\begin{tabular}[c]{@{}c@{}}ElectricTest\\ {\cite{}}\end{tabular}} &
  \multicolumn{1}{l|}{\textbf{Total}} \\ \midrule
\textbf{ET} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{7} \\
\rowcolor{gray!30}
\textbf{GF} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{9} \\
\textbf{MG} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{6} \\
\rowcolor{gray!30}
\textbf{SE} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{6} \\
\textbf{AR} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{6} \\
\rowcolor{gray!30}
\textbf{IT} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{2} \\
\textbf{RO} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{2} \\
\rowcolor{gray!30}
\textbf{LT} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{4} \\
\textbf{FTO} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{2} \\
\rowcolor{gray!30}
\textbf{DC} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{2} \\
\textbf{CTL} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{2} \\
\rowcolor{gray!30}
\textbf{LCM} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{3} \\
\textbf{CI} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{2} \\
\rowcolor{gray!30}
\textbf{RA} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{2} \\
\textbf{ST} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{2} \\
\rowcolor{gray!30}
\textbf{EmT} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{3} \\
\textbf{VT} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{2} \\
\rowcolor{gray!30}
\textbf{TM} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{2} \\
\textbf{DF} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{2} \\
\rowcolor{gray!30}
\textbf{OISS} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{2} \\
\textbf{VHS} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{2} \\
\rowcolor{gray!30}
\textbf{EH} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{2} \\
\textbf{MNT} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{2} \\
\rowcolor{gray!30}
\textbf{RP} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{2} \\
\textbf{UT} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{2} \\
\rowcolor{gray!30}
\textbf{DA} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{2} \\
\textbf{AL} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{2} \\
\rowcolor{gray!30}
\textbf{BA} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{1} \\
\textbf{UI} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{1} \\
\rowcolor{gray!30}
\textbf{InT} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{1} \\
\textbf{DepT} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{1} \\
\rowcolor{gray!30}
\textbf{DT} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{2} \\
\textbf{IgT} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{1} \\
\rowcolor{gray!30}
\textbf{FF} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{0} \\
\textbf{TRW} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
   &
  \textbf{1} \\
\rowcolor{gray!30}
\textbf{OF} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
  &
  \textbf{1} \\
\textbf{PO} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
  &
  \textbf{1} \\
\rowcolor{gray!30}
\textbf{OCT} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
  &
  \textbf{1} \\
\textbf{AT} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
  &
  \textbf{1} \\
\rowcolor{gray!30}
\textbf{LoT} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
  &
  \textbf{1} \\
\textbf{MS} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
  &
  \textbf{1} \\
\rowcolor{gray!30}
\textbf{ConL} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
  &
  \textbf{1} \\
\textbf{AUU} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
  &
  \textbf{1} \\
\rowcolor{gray!30}
\textbf{UMC} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
  &
  \textbf{1} \\
\textbf{USFV} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
  &
  \textbf{1} \\
\rowcolor{gray!30}
\textbf{ERT} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
  &
  \textbf{1} \\
\textbf{MIV} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
  &
  \textbf{1} \\
\rowcolor{gray!30}
\textbf{UCFA} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
  &
  \textbf{1} \\
\textbf{ETMC} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
  &
  \textbf{1} \\
\rowcolor{gray!30}
\textbf{TMC} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
  &
  \textbf{1} \\
\textbf{UCA} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
  &
  \textbf{1} \\
\rowcolor{gray!30}
\textbf{LIOC} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
  &
  \textbf{1} \\
\textbf{UTO} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
  &
  \textbf{1} \\
\rowcolor{gray!30}
\textbf{TOT} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
  &
  \textbf{1} \\
\textbf{TCN} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
  &
  \textbf{1} \\
\rowcolor{gray!30}
\textbf{ESF} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
  &
  \textbf{1} \\
\textbf{TT} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
  &
  \textbf{1} \\
\rowcolor{gray!30}
\textbf{EMC} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
  &
  \textbf{1} \\
\textbf{RA} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
  &
  \textbf{1} \\
\rowcolor{gray!30}
\textbf{COT} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
  &
  \textbf{1} \\
\textbf{GT} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$\surd$} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
  &
  \textbf{1} \\
\rowcolor{gray!30}
\textit{\textbf{Total}} &
  \multicolumn{1}{r|}{\textbf{21}} &
  \multicolumn{1}{r|}{\textbf{19}} &
  \multicolumn{1}{r|}{\textbf{12}} &
  \multicolumn{1}{r|}{\textbf{10}} &
  \multicolumn{1}{r|}{\textbf{6}} &
  \multicolumn{1}{r|}{\textbf{6}} &
  \multicolumn{1}{r|}{\textbf{6}} &
  \multicolumn{1}{r|}{\textbf{5}} &
  \multicolumn{1}{r|}{\textbf{3}} &
  \multicolumn{1}{r|}{\textbf{2}} &
  \multicolumn{1}{r|}{\textbf{26}} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
%  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{--} \\ \bottomrule
\end{tabular}
%
}
\end{table*}

==> Tables/Tool_Table.tex <==

\begin{table*}
\centering
\caption{ List of Test Smell Detection Tools. \wajdi{Precision and recall columns added}}

% \resizebox{\columnwidth}{!}{%
\begin{adjustbox}{width=1.1\textwidth,center}
\begin{threeparttable}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}\hline

\rowcolor{gray!60}
\textbf{No.} & \textbf{Study} & \textbf{Tool Name} & \textbf{\# Test} & \textbf{Detection} & \multicolumn{2}{c|}{\textbf{Programming Language}} & \textbf{Test} & \textbf{Available} & \textbf{Guide} & \textbf{GUI} & \textbf{Precision} & \textbf{Recall} & \textbf{Release} & \textbf{Studies} & \textbf{Tool} \\ \cline{6-7}
\rowcolor{gray!60}
\textbf{} & \textbf{} & \textbf{} & \textbf{Smell} & \textbf{Technique} & \textbf{Developed} & \textbf{Detect} & \textbf{Framework} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{Year} & \textbf{Used the Tool} & \textbf{Link} \\
\hline   


1  & Reichhart et al. \cite{reichhart2007rule}      & TestLint     & 27 & Rule-based/Dynamic analysis* & Smalltalk  & Smalltalk  & Sunit            & Yes          & Yes & N/A & No & No & 2007  & N/A &\cite{TestLint2007} \\ \hline 
\rowcolor{gray!30}
2  & Breugelmans                                    & TestQ        & 12 & Metrics-based  &    Python       & C++        & CppUnit,         & Yes          & Yes & N/A & No & No & 2008  & N/A &\cite{TestQ2008} \\  
\rowcolor{gray!30}
   & \& Rompaey \cite{breugelmans2008testq}         &              &    &          &            & Java       & JUnit, Qtest     &              &     &    &       &   &  &  &  \\ \hline 
   
3  & Bavota et al. \cite{bavota2012empirical}            & Unnamed      & 9  &  Rule-based &     N/A      & Java       & Junit            & No  & No  & N/A & 88\% & 100\% & 2012   & \cite{bavota2015test, tahir2016empirical, palomba2016diffusion, palomba2017does, spadini2018relation, qusef2019exploratory, grano2019scented, palomba2019smell} & \cite{UnnamedTool2014}  \\ \hline 
\rowcolor{gray!30}
4  & Greiler et al. \cite{greiler2013automated}     & TestHound    & 6  & Metrics-based  &      Java     & Java       & Junit, TestNG    & Yes & No  & Yes  & No & No & 2013   & N/A & \cite{TestHound2013} \\ \hline 

5  & Greiler et al. \cite{greiler2013strategies}    & TestEvoHound & 6  &  Metrics-based &     Java      & Java       & Junit, TestNG    & No  & No & N/A & No & No & 2013   & N/A & \cite{TestEvoHound2013} \\ \hline 
\rowcolor{gray!30}
6  & Huo et al. \cite{huo2014improving}             & OraclePolish & 2  &  Dynamic tainting-based &     Java      & Java       & Junit            & Yes & Yes & No  & No & No & 2014   & N/A & \cite{OraclePolish2014}  \\ \hline 

7  & Tufano et al. \cite{tufano2016empirical}       & HistoryMiner & 5  & Rule-based  &  N/A         & Java       & Junit            & No  & N/A  & N/A & No & No & 2016   & N/A & N/A  \\ \hline 
\rowcolor{gray!30}
8  & Palomba et al. \cite{palomba2018automatic}     & TASTE        & 3  &  Information retrieval techniques &   N/A        & Java       & Junit            & No  & No  & N/A & 57\% & 80\% & 2018   & N/A & N/A  \\ \hline 

9  & De Bleser et al. \cite{de2019assessing}        & SOCRATES     & 6  & Rule-based  & Scala      & Scala      & ScalaTest        & Yes & Yes & Yes & 98.94\% & 89.59\% & 2019   & \cite{de2019socrates} & \cite{SOCRATES2019}  \\ \hline 
\rowcolor{gray!30}
10 & Peruma et al. \cite{peruma2019distribution}    & \textsc{tsDetect}     & 19 &  Rule-based & Java       & Java       & Junit            & Yes & Yes & No & 85\%-100\% & 90\%-100\% & 2019   & \cite{schvarcbacher2019investigating} & \cite{tsDetect2019}  \\ \hline 
11 & Virginio et al. \cite{virginio2019influence}   & JNose        & 21 &  Rule-based & Java       & Java       & Junit            & Yes & Yes & Yes & No & No & 2019   & N/A & \cite{JNose2019}  \\ \hline 

\end{tabular}
\begin{tablenotes}
            \item[*] The tool integrates dynamic analysis for specific smells  \cite{greiler2013automated}.
        \end{tablenotes}
\end{threeparttable}

\end{adjustbox}
% }
%{\raggedright \textbf{Note:} The studies\cite{van2007detection, van2006characterizing} did not mention the tools they used in their researches.  \par}

\label{tab:Tools_Table}
\end{table*}

==> Tables/Tool_Table_v2.tex <==
\begin{table*}
\centering
\caption{Feature availability of test smell detection tools.}
\label{tab:Tools_Table_v2}

\resizebox{\textwidth}{!}{%
\begin{threeparttable}

\begin{tabular}{|llllllllll|}

\rowcolor{gray!60}
\multicolumn{1}{|c}{\cellcolor{gray!60}} &
  \multicolumn{2}{c}{\cellcolor{gray!60}\textbf{Programming Language}} &
  \multicolumn{1}{c}{\cellcolor{gray!60}} &
  \multicolumn{2}{c}{\cellcolor{gray!60}\textbf{Correctness}} &
  \multicolumn{1}{c}{\cellcolor{gray!60}} &
  \multicolumn{1}{c}{\cellcolor{gray!60}} &
  \multicolumn{1}{c}{\cellcolor{gray!60}} &
  \multicolumn{1}{c|}{\cellcolor{gray!60}} \\
\rowcolor{gray!60}
\multicolumn{1}{|c}{\multirow{-2}{*}{\cellcolor{gray!60}\textbf{Tool}}} &
  \multicolumn{1}{c}{\cellcolor{gray!60}\textbf{Implemented}} &
  \multicolumn{1}{c}{\cellcolor{gray!60}\textbf{Analyzed}} &
  \multicolumn{1}{c}{\multirow{-2}{*}{\cellcolor{gray!60}\textbf{\begin{tabular}[c]{@{}c@{}}Supported \\      Test Framework\end{tabular}}}} &
  \multicolumn{1}{c}{\cellcolor{gray!60}\textbf{Precision}} &
  \multicolumn{1}{c}{\cellcolor{gray!60}\textbf{Recall}} &
  \multicolumn{1}{c}{\multirow{-2}{*}{\cellcolor{gray!60}\textbf{\begin{tabular}[c]{@{}c@{}}Detection \\ Technique\end{tabular}}}} &
  \multicolumn{1}{c}{\multirow{-2}{*}{\cellcolor{gray!60}\textbf{\begin{tabular}[c]{@{}c@{}}Useage Guide\\ Availability\end{tabular}}}} &
  \multicolumn{1}{c}{\multirow{-2}{*}{\cellcolor{gray!60}\textbf{Research Citations}}} &
  \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor{gray!60}\textbf{Availability}}} \\ \hline
\textbf{JNose Test} \cite{virginio2020jnose} &
  Java &
  Java &
  JUnit &
  UNK &
  UNK &
  Rule-based &
  Yes &
  \cite{virginio2019influence, virginio2020empirical} &
  \cite{Download:JNose2019}  \\
\rowcolor{gray!30}
\textbf{\textsc{tsDetect}} \cite{peruma2020FSE} &
  Java &
  Java &
  JUnit &
  85\%-100\% &
  90\%-100\% &
  Rule-based &
  Yes &
  \cite{peruma2019CASCON,schvarcbacher2019investigating,Spadini2020MSR,Kim2020ICSE,Fraser2020ICSTW,Panichella2020ICSME,Soares2020SAST,Peruma2020IWoR, spadini2020investigating} &
  \cite{Download:tsDetect2019} \\
\textbf{TestQ} \cite{breugelmans2008testq} &
  Python &
  C++, Java &
  CppUnit, JUnit,   Qtest &
  UNK &
  UNK &
  Metrics-based &
  Yes &
  -- &
  \cite{Download:TestQ2008} \\
\rowcolor{gray!30}
\textbf{Unnamed} \cite{bavota2012empirical} &
  UNK &
  Java &
  JUnit &
  88\% &
  100\% &
  Rule-based &
  No &
  \cite{bavota2015test, tahir2016empirical, palomba2016diffusion, palomba2017does, spadini2018relation, qusef2019exploratory, grano2019scented, palomba2019smell, Panichella2020ICSME}  &
  UNK \\
\textbf{TestHound} \cite{greiler2013automated} &
  Java &
  Java &
  JUnit, TestNG &
  UNK &
  UNK &
  Metrics-based &
  No &
  -- &
  \cite{Download:TestHound2013} \\
\rowcolor{gray!30}
\textbf{TestEvoHound} \cite{greiler2013strategies} &
  Java &
  Java &
  JUnit, TestNG &
  UNK &
  UNK &
  Metrics-based &
  No &
  -- &
  UNK  \\
\textbf{SoCRATES} \cite{de2019socrates} &
  Scala &
  Scala &
  ScalaTest &
  98.94\% &
  89.59\% &
  Rule-based &
  Yes &
  \cite{de2019socrates}  &
  \cite{Download:SOCRATES2019} \\
\rowcolor{gray!30}
\textbf{HistoryMiner} \cite{tufano2016empirical} &
  UNK &
  Java &
  JUnit &
  UNK &
  UNK &
  Rule-based &
  No &
  -- &
  UNK \\
\textbf{TASTE} \cite{palomba2018automatic} &
  UNK &
  Java &
  JUnit &
  57\%-75\% &
  60\%-80\% &
  Information retrieval-based &
  No &
  -- &
  UNK \\
\rowcolor{gray!30}
\textbf{OraclePolish} \cite{huo2014improving} &
  Java &
  Java &
  JUnit &
  UNK &
  UNK &
  Dynamic tainting-based &
  Yes &
  -- &
  \cite{Download:OraclePolish2014} \\
\textbf{TestLint} \cite{reichhart2007rule} &
  Smalltalk &
  Smalltalk &
  Sunit &
  UNK &
  UNK &
  Rule-\&, Dynamic tainting-based &
  Yes &
  -- &
  \cite{Download:TestLint2007} \\ 
\rowcolor{gray!30}
\textcolor{red}{  \textbf{RAIDE*} }\cite{Santana2020SBES} &
  Java &
  Java &
  JUnit &
  UNK &
  UNK &
  Rule-based &
  Yes &
  -- &
  \cite{Download:RAIDE2020} \\ 
  \textcolor{red}{  \textbf{DARTS*} }\cite{lambiase2020just} &
  Java &
  Java &
  JUnit &
  UNK &
  UNK &
  Information retrieval-based &
  Yes &
  -- &
  \cite{Download:DARTS2020} \\ 
\rowcolor{gray!30}
\textcolor{red}{  \textbf{DTDetector}} \cite{zhang2014empirically} &
  Java &
  Java &
  JUnit &
  UNK &
  UNK &
  Dynamic tainting-based &
  Yes &
  \textcolor{red}{TBD} &
  \cite{Download:DTDetector} \\ 
\textcolor{red}{ \textbf{TeCReVis}} \cite{koochakzadeh2010tecrevis} &
  Java &
  Java &
  JUnit &
  UNK &
  UNK &
  Metrics-\&, Dynamic tainting-based  &
  Yes &
  \textcolor{red}{TBD} &
  UNK \\
\rowcolor{gray!30}
\textcolor{red}{ \textbf{TeReDetect}} \cite{koochakzadeh2010tester} &
  Java &
  Java &
  JUnit &
  UNK &
  UNK &
  Metrics-\&, Dynamic tainting-based &
  No &
  \textcolor{red}{TBD} &
  UNK \\ 
\textcolor{red}{ \textbf{TRex*}} \cite{baker2006trex} &
  Java &
  Java &
  TTCN-3 &
  UNK &
  UNK &
  Rule-based &
  Yes &
  \textcolor{red}{TBD} &
  \cite{Download:TRex} \\
\rowcolor{gray!30}
  \textcolor{red}{ \textbf{POLDET}} \cite{gyori2015reliable} &
  Java &
  Java &
  JUnit &
  UNK &
  UNK &
  Dynamic tainting-based &
  No &
  \textcolor{red}{TBD} &
  UNK \\ 
  \textcolor{red}{ \textbf{TEDD}} \cite{biagiola2019web} &
  Java &
  Java &
  JUnit &
  80\% &
  94\% &
  Information retrieval-based &
  Yes &
  \textcolor{red}{TBD} &
  \cite{Download:TEDD} \\ 
\rowcolor{gray!30}
  \textcolor{red}{ \textbf{PRADET}} \cite{gambi2018practical} &
  Java &
  Java &
  JUnit &
  UNK &
  UNK &
  Dynamic tainting-based &
  Yes &
  \textcolor{red}{TBD} &
  \cite{Download:Pradet2018} \\  
  \textcolor{red}{ \textbf{ElectricTest}} \cite{bell2015efficient} &
  Java &
  Java &
  JUnit &
  UNK &
  UNK &
  Dynamic tainting-based  &
  No &
  \textcolor{red}{TBD} &
  UNK \\  
  
  \hline
  
\end{tabular}%
\begin{tablenotes}
            \item[*] The tool also provides support for refactoring.
        \end{tablenotes}
\end{threeparttable}
}
\end{table*}

==> Tables/VenueTable.tex <==
\begin{table*}[ht]
\resizebox{\textwidth}{!}{%
% \begin{adjustbox}{width=1.0\textwidth,center}
\begin{tabular} {cllcc}
\hline
% \toprule

\rowcolor{gray!60}
\textbf{No.} & \textbf{Venue} & \textbf{Type}  & \textbf{\# of Studies} & \textbf{Ref}\\ \hline     

\textbf{1} &  International Conference on Software Maintenance and Evolution (ICSME)                  &   Conference  &   3 &  \cite{palomba2017does, palomba2018automatic, spadini2018relation}  \\  \hline
%%%%%
\rowcolor{gray!30}
\textbf{2} &  International Conference on Mining Software Repositories (MSR)                          &   Conference  &   2 &  \cite{de2019assessing, greiler2013strategies}  \\  \hline
%%%%%
\textbf{3} &  International Conference on Software Maintenance (ICSM)                                 &   Conference  &   2 &  \cite{bavota2012empirical, van2006characterizing}  \\  \hline
%%%%%
\rowcolor{gray!30}
\textbf{4} &  Empirical Software Engineering                                                          &   Journal     &   2 &   \cite{bavota2015test, palomba2019smell} \\  \hline
%%%%%
\textbf{5} &  Journal of Systems and Software (JSS)                                                   &   Journal     &   1 &   \cite{grano2019scented} \\  \hline
%%%%%
\rowcolor{gray!30}
\textbf{6} & International Conference on Computer Science and Software Engineering (CASCON)           &   Conference  &   1 &  \cite{peruma2019distribution}  \\  \hline
%%%%%
\textbf{7} &  Brazilian Symposium on Software Engineering (SBES)                                      &   Symposium   &   1 &  \cite{virginio2019influence}  \\  \hline
%%%%%
\rowcolor{gray!30} 
\textbf{8} &  IEEE Access                                                                             &   Journal     &   1 &  \cite{qusef2019exploratory}  \\  \hline
%%%%%
\textbf{9} &  International Conference on Software Testing, Verification and Validation (ICST)        &   Conference  &   1 &  \cite{greiler2013automated}  \\  \hline
%%%%%
\rowcolor{gray!30}
\textbf{10} &  Journal of Object Technology                                                           &   Journal     &   1 &  \cite{reichhart2007rule}  \\  \hline
%%%%%
\textbf{11} &  International Conference on Automated Software Engineering (ASE)                       &   Conference  &   1 &  \cite{tufano2016empirical}  \\  \hline
%%%%%
\rowcolor{gray!30}
\textbf{12} &  Transactions on Software Engineering (TSE)                                             &   Journal     &   1 &  \cite{van2007detection}  \\  \hline
%%%%%
\textbf{13} &  International Symposium on Foundations of Software (FSE)                               &   Conference  &   1 &   \cite{huo2014improving} \\  \hline
%%%%%
\rowcolor{gray!30} 
\textbf{14} &  International Workshop on Search-Based Software Testing (SBST)                         &   Workshop    &   1 &  \cite{palomba2016diffusion}  \\  \hline
%%%%%
\textbf{15} &  Scala Symposium                                                                        &   Symposium   &   1 &  \cite{de2019socrates}  \\  \hline
%%%%%
\rowcolor{gray!30}
\textbf{16} &  Advanced Techniques Tools for Software Evolution (SATTOSE)                             &   Seminar     &   1 &   \cite{schvarcbacher2019investigating} \\  \hline
%%%%%
\textbf{17} &  Asia-Pacific Software Engineering Conference (APSEC)                                   &   Conference  &   1 &   \cite{tahir2016empirical} \\  \hline
%%%%%
\rowcolor{gray!30} 
\textbf{18} &  International Workshop on Advanced Software Development Tools and Techniques (WASDeTT) &   Workshop    &   1 & \cite{breugelmans2008testq}   \\  
%%%%%


\hline

\end{tabular}

% \end{adjustbox}
}
\caption{Information .}
\label{tab:DatasetContent}

\end{table*}
